Reducing CMSO Model Checking to Highly Connected Graphs

Given a Counting Monadic Second Order (CMSO) sentence $\psi$, the CMSO$[\psi]$ problem is defined as follows. The input to CMSO$[\psi]$ is a graph $G$, and the objective is to determine whether $G\models \psi$. Our main theorem states that for every CMSO sentence $\psi$, if CMSO$[\psi]$ is solvable in polynomial time on "globally highly connected graphs", then CMSO$[\psi]$ is solvable in polynomial time (on general graphs). We demonstrate the utility of our theorem in the design of parameterized algorithms. Specifically we show that technical problem-specific ingredients of a powerful method for designing parameterized algorithms, recursive understanding, can be replaced by a black-box invocation of our main theorem. We also show that our theorem can be easily deployed to show fixed parameterized tractability of a wide range of problems, where the input is a graph $G$ and the task is to find a connected induced subgraph of $G$ such that "few" vertices in this subgraph have neighbors outside the subgraph, and additionally the subgraph has a CMSO-definable property.

==> content.tex <==
\section{???}

\subsection{The {\sc CMSO}[$\psi]$ Problem}\label{sec:prob}

\hly{todo}

\subsection{???}

\begin{theorem}\label{thm:main}
Let $\psi$ be a CMSO sentence. For all $c,d\in\mathbb{N}$, if there exist $s\in\mathbb{N}$ and an algorithm that solves {\sc CMSO}$[\psi]$ on $(s,c)$-unbreakable structures in time $\OO(n^d)$, then there exists an algorithm that solves {\sc CMSO}$[\psi]$ on general structures in time $\OO(n^{d+?})$.\hly{Fill the `?'.}
\end{theorem}

